LocCa: Visual Pretraining with Location-aware Captioners

Image captioning has been shown as an effective pretraining method similar to contrastive pretraining. However, the incorporation of location-aware information into visual pretraining remains an area with limited research. In this paper, we propose a simple visual pretraining method with location-aware captioners (LocCa). LocCa uses a simple image captioner task interface, to teach a model to read out rich information, i.e. bounding box coordinates, and captions, conditioned on the image pixel input. Thanks to the multitask capabilities of an encoder-decoder architecture, we show that an image captioner can easily handle multiple tasks during pretraining. Our experiments demonstrate that LocCa outperforms standard captioners significantly on localization downstream tasks while maintaining comparable performance on holistic tasks.

==> tbls/coco_det.tex <==
\begin{table}[!t]
\centering
\caption{Result on COCO detection with res=640 and a limit of 25 output boxes. For reward tuned models we show both the result before and after. O365 indicates the results when initializing both the encoder and decoder with the objects365 pretrained model.}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{lcc}
\hline
\textbf{MODEL} & \textbf{mAP (\%)} & \textbf{AR (\%)} \\
\hline
Pix2seq$_{\mathrm{res=}1280}$\cite{chen2022pixseq} & 47.1 & N/A \\
O365$_{\mathrm{res=640}}$ & 34.8 $\rightarrow$ 49.4 & 50.0 $\rightarrow$ 59.4 \\ 
Con & 28.1 $\rightarrow$ 40.5 & 40.9 $\rightarrow$ 48.5 \\
Cap & 25.3 $\rightarrow$ 39.0 & 39.2 $\rightarrow$ 48.7 \\
CapPa & 25.1 $\rightarrow$ 39.5 & 39.6 $\rightarrow$ 48.8 \\
\modelname{} & 33.2 $\rightarrow$ 47.7 & 48.3 $\rightarrow$ 56.3 \\
\hline
\modelname{}$_{\mathrm{decoder=from\ scratch}}$ & 25.3 $\rightarrow$ x & 39.6 $\rightarrow$ x \\
\modelname{}$_{\mathrm{res=640}}$ & 35.1 $\rightarrow$ 48.7 & 49.7 $\rightarrow$ 57.1 \\

\hline
\end{tabular}}
\label{tbl:coco_det}
\end{table}


==> tbls/dup_ids.tex <==
154, 309, 605, 656, 716, 797, 839, 909, 977, 1298, 1488, 1507, 1947, 1958, 1994, 2083, 2342, 2400, 2411, 2448, 2567, 2742, 2843, 2964, 3000, 3178, 3293, 3518, 3751, 4244, 4424, 4477, 4587, 5152, 5377, 5424, 5434, 5508, 5614, 5632, 5862, 5962, 6026, 6051, 6407, 6747, 6842, 6943, 6964, 7028, 7145, 7277, 7393, 7476, 7504, 7601, 7621, 7944, 7945, 7946, 8063, 8300, 8320, 8429, 8936, 9017, 9018, 9029, 9057, 9218, 9723, 9822, 10094, 10179, 10229, 10471, 10710, 10948, 11065, 11282, 11324, 11774, 12224, 12377, 12382, 12440, 12495, 12614, 12790, 13352, 13576, 13670, 13763, 13856, 14008, 14025, 14160, 14283, 14468, 14484, 14502, 14864, 15190, 15195, 15554, 15809, 16089, 16273, 16465, 16616, 16659, 16669, 16725, 16796, 16814, 16836, 16870, 17236, 17468, 17566, 17587, 17938, 17997, 18075, 18089, 18093, 18211, 18244, 18370, 18542, 18780, 19123, 19374, 19501, 19789, 19959, 19967, 20044, 20156, 20188, 20279, 20513, 20619, 20917, 21292, 21504, 21750, 21830, 22102, 22195, 22222, 22287, 22575, 22740, 22928, 23014, 23141, 23194, 23420, 23538, 23967, 24038, 24086, 24129, 24404, 24689, 24706, 24762, 24842, 24939, 25237, 25353, 25414, 25515, 25628, 26052, 26421, 26438, 26583, 26997, 27070, 27149, 27424, 27495, 27750, 27763, 28012, 28038, 28069, 28154, 28281, 28451, 28560, 28824, 28974, 28988, 29304, 29456, 29473, 29601, 29752, 29799, 30203, 30274, 30340, 30418, 30631, 30973, 31112, 31187, 31230, 31329, 31374, 31382, 31418, 31838, 32061, 32105, 32289, 33017, 33527, 33572, 33991, 33992, 34223, 34616, 34739, 34810, 35045, 35132, 35230, 35265, 35322, 35473, 35558, 35571, 35796, 36017, 36445, 36488, 36546, 36755, 36981, 37089, 37282, 37429, 37539, 37582, 37698, 37719, 37800, 37847, 37862, 38033, 38266, 38552, 38890, 39159, 39185, 39258, 39629, 39802, 39812, 40130, 40346, 40735, 41713, 41730, 41818, 41988, 42696, 42804, 43163, 43609, 43655, 43664, 43813, 43892, 44123, 44266, 44298, 44637, 44901, 44960, 45226, 45464, 45659, 45672, 45840, 46055, 46385, 46519, 46609, 46809, 47093, 47175, 47198, 47294, 47347, 47357, 47391, 47451, 47554, 47774, 47928, 48267, 48432, 48572, 48665, 48707, 48937, 49022, 49073, 49866, 50105, 50134, 50161, 50601, 50961, 51001, 51052, 51550, 51563, 51706, 51835, 51965, 52109, 52168, 52219, 52448, 52484, 52626, 52729, 52751, 52929, 53004, 53232, 53304, 53335, 53370, 53388, 53601, 53928, 53929, 54402, 54541, 54572, 54764, 54805, 54806, 55226, 55232, 55385, 55733, 55764, 55873, 56028, 56032, 56604, 56616, 56632, 56667, 56699, 56738, 57551, 57689, 57699, 57828, 57870, 58184, 58403, 58633, 58836, 59079, 59231, 59382, 59483, 59556, 59593, 59654, 59816, 59947, 60043, 60155, 60182, 60639, 61159, 61328, 61372, 61459, 61460, 61842, 61843, 61936, 62038, 62057, 62131, 62203, 62233, 62263, 62455, 62477, 62759, 63084, 63238, 63334, 63337, 63347, 63754, 63820, 63867, 64317, 64392, 64962, 65011, 65136, 65769, 65841, 65842, 66236, 66518, 66566, 66593, 66637, 66737, 67356, 67438, 67615, 67748, 68139, 68397, 68430, 68459, 68786, 69047, 69344, 69432, 69488, 69971, 69978, 70000, 70094, 70161, 70415, 70718, 70745, 70755, 71099, 71229, 71271, 71399, 71714, 71970, 71989, 72111, 72396, 72565, 72592, 72629, 72731, 72947, 72995, 73174, 73583, 73591, 73602, 73610, 73671, 73680, 73999, 74127, 74156, 74201, 74215, 74577, 74663, 74925, 74942, 74945, 74996, 75590, 75691, 75843, 75881, 75924, 76245, 76414, 76590, 76781, 76882, 76885, 77005, 77174, 77332, 77377, 77380, 77417, 78009, 78221, 78274, 78425, 78482, 78536, 78572, 79083, 79313, 79441, 79456, 79611, 79701, 79783, 79887, 80207, 80305, 80472, 80521, 80634, 80782, 80818, 80835, 81065, 81128, 81200, 81283, 81372, 81768, 81799, 81810, 82083, 82228, 82484, 83005, 83353, 83448, 83725, 83815, 83866, 84162, 84167, 84259, 84558, 84594, 84712, 84800, 84803, 85549, 85893, 85960, 86075, 86216, 86217, 86459, 86549, 86654, 86750, 86754, 86869, 87214, 87235, 87458, 87522, 87569, 87671, 87737, 87792, 88200, 88609, 88653, 88671, 88726, 88868, 89005, 89181, 89187, 89208, 89651, 89734, 89788, 89882, 89902, 89921, 89931, 90277, 90310, 90350, 90444, 90569, 90573, 90830, 90985, 91055, 91056, 91130, 91288, 91784, 92009, 92165, 92439, 92480, 92646, 92685, 92694, 93171, 93531, 93581, 93786, 93885, 94459, 94618, 94826, 95061, 95257, 95518, 95562, 95676, 95812, 96177, 96244, 96338, 96475, 96728, 96808, 96859, 96958, 97411, 97563, 97795, 97818, 98447, 99040, 99159, 99211, 99293, 99451, 99727, 100182, 100209, 100485, 100586, 100722, 100777, 101479, 101503, 101573, 101697, 101807, 101832, 101882, 101891, 102144, 102208, 102281, 102290, 102662, 102667, 103223, 103251, 103419, 103510, 104126, 104248, 104277, 104304, 104344, 104410, 104692, 104752, 105026, 105063, 105219, 105470, 105660, 105714, 105719, 105859, 106100, 106148, 106315, 106383, 106557, 106832, 106978, 106994, 107009, 107100, 107156, 107767, 107846, 108375, 108499, 108920, 109088, 109553, 109654, 109778, 109895, 110230, 110252, 110447, 110989, 111040, 111045, 111195, 111543, 111705, 111754, 111842, 111992, 112040, 112226, 112495, 112577, 112707, 113032, 113123, 113152, 113244, 113676, 113844, 113998, 114060, 114326, 114459, 114786, 114801, 114807, 115505, 115524, 115564, 116040, 116049, 116603, 116607, 116824, 116832, 116882, 117117, 117182, 117447, 117578, 117677, 117772, 117969, 118169, 118277, 118413, 118543, 118697, 118780, 118827, 119093, 119129, 119263, 119534, 119543, 119714, 119974, 120155, 120274, 120333, 120431, 120836, 121445, 121453, 121575, 121619, 121683, 121903, 121938, 121965, 121994, 122099, 122259, 122436, 122459, 122916, 122918, 123180, 123366, 124030, 124055, 124069, 124169, 124178, 124694, 124711, 124751, 124786, 124804, 125658, 125690, 125774, 125785, 125882, 126381, 126447, 126534, 126737, 126825, 126909, 127282, 127316, 127388, 127543, 127560, 127615, 127629, 127729, 127945, 128106, 128127, 128136, 128282, 128385, 128434, 128475, 128599, 128647, 128775, 129438, 129551, 129771, 129806, 130116, 130163, 130215, 130324, 130339, 130518, 130872, 131058, 131074, 131127, 131277, 131449, 131587, 131595, 131816, 132183, 132529, 132574, 132585, 132617, 132746, 133295, 133384, 133609, 133654, 133905, 133940, 134100, 134176, 134420, 134447, 134474, 134755, 134799, 135332, 135482, 135539, 135694, 135815, 135822, 136092, 136230, 136232, 136310, 136331, 136563, 136736, 136811, 137052, 137378, 137516, 137715, 137724, 137730, 137918, 138131, 138436, 138507, 138567, 138910, 139068, 139173, 139324, 139359, 139429, 139568, 139696, 139728, 139763, 139775, 139811, 139914, 140053, 140108, 140291, 140733, 140738, 140850, 140954, 141101, 141603, 141682, 141702, 141827, 141952, 142322, 142431, 142439, 142969, 143003, 143258, 143323, 143334, 143470, 143665, 144272, 144275, 144320, 144495, 144519, 144574, 144817, 144832, 144851, 144906, 145178, 145180, 145192, 146561, 147466, 147701, 147710, 147733, 147753, 147760, 147838, 148044, 148047, 148809, 148937, 149180, 149202, 149253, 149498, 149556, 149566, 149616, 149916, 150044, 150100, 150477, 150614, 150704, 151163, 151178, 151236, 151265, 151523, 151699, 151756, 151908, 152003, 152197, 152237, 152238, 152273, 152501, 152556, 152871, 152954, 153340, 153475, 153591, 153671, 153749, 153814, 153845, 154244, 154713, 154895, 154911, 155107, 155268, 155269, 155379, 155549, 155860, 155904, 156125, 156258, 156608, 156757, 156823, 156827, 156914, 156939, 157125, 157194, 157242, 157344, 157424, 157714, 157744, 157834, 157926, 158051, 158201, 158362, 158686, 158701, 159038, 159682, 159768, 159957, 160101, 160291, 160503, 160614, 160648, 160688, 160852, 161719, 161818, 161865, 162046, 162102, 162283, 162300, 162551, 162645, 162760, 163054, 163089, 163266, 163394, 163559, 163598, 163991, 164043, 164100, 164381, 164855, 164935, 165077, 165199, 165555, 165868, 166073, 166230, 166328, 166653, 166762, 167169, 167264, 167755, 167765, 168022, 168179, 168366, 168482, 168643, 168865, 169179, 169529, 169656, 169725, 170327, 170398, 170483, 170623, 170636, 170683, 170689, 170712, 170809, 170976, 170980, 171262, 171478, 171536, 171729, 171943, 172669, 172957, 173032, 173056, 173484, 173538, 173550, 173814, 173925, 174059, 174137, 174554, 174700, 174749, 174774, 174876, 174892, 175112, 175116, 175118, 175162, 175195, 175284, 175405, 175480, 175523, 175881, 176008, 176032, 176229, 176342, 176386, 176790, 176810, 176871, 177019, 177193, 177289, 177314, 177353, 177472, 177516, 177817, 177821, 177915, 177917, 178131, 178192, 178492, 178763, 178874, 178987, 179011, 179164, 179390, 179618, 179763, 179969, 180179, 180220, 180285, 180354, 180559, 180578, 180667, 181054, 181176, 181475, 181681, 181929, 182406, 182505, 182571, 182642, 182863, 183022, 183236, 183237, 183392, 183435, 183538, 183626, 183646, 183653, 183788, 183835, 183923, 184106, 184184, 184513, 185153, 185258, 186131, 186198, 186246, 186255, 186336, 186605, 187147, 187511, 187939, 188087, 188184, 188587, 188621, 188845, 188911, 189330, 189353, 189646, 189924, 190026, 190216, 190219, 190277, 190513, 190617, 190732, 191068, 191305, 191327, 191561, 191754, 192301, 192319, 192407, 192476, 192524, 192878, 193042, 193168, 193171, 193682, 193829, 194056, 194154, 194193, 194438, 194448, 194550, 194669, 194677, 194679, 194726, 194758, 194847, 195027, 195188, 195525, 195861, 196111, 196112, 196156, 196170, 196198, 196653, 196971, 197222, 197251, 197323, 197401, 197525, 197591, 197663, 198277, 198651, 198785, 199234, 199331, 199485, 199835, 199836, 199888, 199963, 200010, 200181, 200377, 200404, 201184, 201322, 201634, 201897, 202657, 202755, 203034, 203036, 203098, 203108, 203175, 203458, 203459, 203994, 204053, 204294, 204759, 204792, 204800, 205000, 205131, 205202, 205223, 205250, 205460, 205794, 205963, 206377, 206486, 206628, 206731, 206968, 207381, 207467, 207496, 207629, 208075, 208379, 208396, 208724, 208845, 208963, 209089, 209185, 209191, 209356, 209449, 209537, 209563, 209603, 209654, 209844, 209993, 210187, 210252, 210271, 210279, 210604, 210710, 210773, 210848, 211138, 211570, 211576, 211683, 212070, 212247, 212450, 212532, 212628, 212635, 212641, 212757, 212974, 213408, 213419, 213426, 214523, 214875, 215026, 215191, 215201, 215243, 215357, 215407, 215421, 215563, 215701, 215908, 216391, 216579, 216676, 216840, 217043, 217151, 217276, 217429, 217487, 217799, 217893, 217959, 217978, 218057, 218096, 218145, 218579, 218734, 218984, 219127, 219248, 219349, 219535, 219680, 219966, 220037, 220053, 220148, 220485, 220504, 220529, 221053, 221169, 221187, 221252, 221625, 221674, 221794, 221880, 221889, 222113, 222209, 222676, 222977, 223023, 223078, 223165, 223270, 223603, 223650, 223790, 223831, 223909, 224056, 224060, 224168, 224541, 224692, 224734, 224753, 224821, 224838, 225069, 225468, 225539, 225579, 225604, 225641, 225755, 226102, 226176, 226329, 226348, 226357, 226460, 226552, 226681, 226712, 226734, 226817, 226961, 226966, 227198, 227205, 227520, 227554, 228000, 228119, 228133, 229041, 229105, 229193, 229362, 229415, 229422, 229598, 229678, 229825, 230436, 230515, 230545, 230559, 230570, 230893, 231047, 231087, 231337, 231992, 232371, 232770, 233007, 233022, 233071, 233153, 233642, 233841, 233871, 233878, 234244, 234653, 234699, 234819, 235468, 235582, 235802, 236036, 236174, 236381, 236397, 236556, 236718, 236961, 237110, 237137, 237193, 237273, 237340, 237355, 237367, 237510, 237834, 237922, 237976, 238007, 238070, 238187, 238231, 238238, 238502, 238618, 238630, 238667, 238713, 239263, 239461, 239559, 239596, 239654, 239772, 239933, 240225, 240331, 240339, 240378, 240500, 240521, 240586, 240662, 240945, 241369, 241887, 242076, 242090, 242145, 242213, 242350, 242453, 242506, 242583, 242709, 242745, 242807, 242854, 243071, 243153, 243336, 243574, 243717, 243824, 243839, 243959, 244016, 244171, 244387, 244425, 244528, 244616, 244825, 244836, 244839, 244844, 244846, 244875, 244983, 245118, 245326, 245946, 246084, 246089, 246342, 246356, 246539, 246641, 246753, 246777, 246959, 247082, 247110, 247265, 247271, 247368, 247660, 247979, 248052, 248337, 248579, 248640, 248666, 248730, 248733, 248835, 248932, 248957, 248979, 249805, 250293, 250295, 250569, 251368, 251523, 251868, 252025, 252136, 252373, 252492, 252768, 252937, 253064, 253087, 253229, 253251, 253335, 253430, 253796, 253834, 254577, 254821, 255203, 256190, 256215, 256364, 256659, 256930, 256951, 257301, 257392, 257451, 257576, 257804, 257815, 257867, 257874, 258165, 258237, 258249, 258505, 258571, 258705, 259120, 259375, 259484, 259514, 259595, 259655, 259809, 260029, 260118, 260181, 260206, 260299, 260317, 260360, 260448, 260668, 260932, 260957, 261283, 261503, 261521, 261673, 261696, 261720, 261990, 262031, 262180, 262239, 262528, 263039, 263176, 263420, 263516, 263924, 264016, 264058, 264165, 264502, 264567, 264741, 264781, 264846, 264885, 265292, 265329, 265625, 265713, 265766, 265980, 266207, 266228, 266240, 266442, 266515, 266816, 266859, 266898, 267049, 267189, 267779, 267794, 267815, 267851, 267898, 267907, 268260, 268428, 268644, 268726, 268881, 268897, 269160, 269199, 269245, 269380, 269504, 269605, 269890, 270111, 270391, 270696, 270844, 271106, 271447, 271641, 272022, 272058, 272235, 272255, 272299, 272310, 272670, 272716, 272729, 272773, 273197, 274139, 274275, 274499, 274642, 274667, 274770, 274786, 274839, 274853, 274986, 275544, 275556, 275658, 275707, 275709, 275775, 275811, 275917, 275932, 276089, 276244, 276354, 276417, 276621, 276666, 276686, 276711, 276740, 276845, 276874, 277202, 277267, 277418, 277439, 277507, 278461, 278931, 279076, 279377, 279485, 279530, 279762, 279882, 280018, 280156, 280191, 280257, 281051, 281237, 281464, 281790, 282067, 282142, 282310, 282514, 282568, 283263, 283479, 283573, 283666, 283673, 283937, 284348, 284639, 284778, 284934, 284964, 285000, 285064, 285093, 285170, 285214, 285307, 285395, 285529, 285548, 286000, 286051, 286132, 286190, 286359, 286411, 286469, 286745, 287140, 287249, 287302, 287567, 287718, 288559, 288610, 288943, 289140, 289282, 289696, 289782, 289791, 289866, 290072, 290098, 290114, 290185, 290265, 290354, 290370, 290549, 290620, 290938, 291039, 291366, 291526, 291897, 292116, 292271, 292386, 292498, 292558, 292751, 293293, 293311, 293489, 293853, 293966, 294409, 295370, 295578, 295759, 295940, 296093, 296191, 296267, 296360, 296474, 296614, 296635, 296747, 296760, 296894, 296984, 297011, 297019, 297251, 297266, 297360, 297363, 297527, 297665, 297764, 297984, 297997, 298110, 298160, 298312, 298360, 298639, 298793, 298931, 298956, 298983, 299029, 299041, 299051, 299085, 299122, 299123, 299463, 299594, 299859, 299933, 299959, 300021, 300197, 300239, 300624, 301109, 301158, 301218, 301413, 301461, 301943, 301970, 301988, 302199, 302353, 302397, 302415, 302885, 303144, 303247, 303360, 303541, 303923, 304092, 304125, 304319, 304406, 304603, 304833, 305105, 305106, 305141, 305219, 305231, 305267, 305492, 305546, 305550, 305564, 305624, 306275, 306393, 306485, 306837, 306967, 307082, 307190, 307242, 307322, 307475, 307671, 307757, 307881, 307968, 308089, 308139, 308210, 308265, 308524, 309034, 309084, 309135, 309280, 309400, 309409, 309706, 310006, 310158, 310360, 310457, 310518, 310759, 310780, 310851, 310865, 310897, 311273, 311388, 311620, 311709, 311773, 311890, 311933, 312154, 312205, 312247, 312282, 312390, 312454, 312608, 312748, 312785, 312886, 312943, 313071, 313073, 313164, 313206, 313209, 313360, 313518, 313569, 313724, 313786, 313873, 313946, 313950, 314065, 314237, 314254, 314319, 314462, 314734, 314920, 314951, 315411, 315555, 315581, 315751, 315944, 315961, 316170, 316293, 316446, 316671, 316801, 316971, 317054, 317349, 317391, 317659, 317805, 317905, 318117, 318183, 318203, 318528, 318953, 319062, 319192, 319396, 319543, 319644, 319685, 319735, 319866, 320059, 320077, 320125, 320137, 320292, 320308, 320371, 320390, 320403, 320611, 320667, 320721, 320834, 320957, 321305, 321673, 321766, 321960, 321969, 322090, 322411, 322630, 322634, 322698, 322726, 323052, 323147, 323149, 323213, 323240, 323389, 323664, 323722, 323728, 323734, 323960, 324528, 324677, 324732, 324910, 325229, 325302, 325362, 325494, 325548, 325950, 326092, 326237, 326357, 326475, 326836, 326841, 326966, 327132, 327198, 327209, 327258, 327338, 327404, 327561, 327694, 327843, 327970, 327998, 328113, 328214, 328298, 328663, 328855, 328917, 329058, 329141, 329343, 329501, 329502, 329528, 329616, 329724, 329963, 329993, 330040, 330094, 330223, 330284, 330342, 330671, 330716, 330752, 330785, 330991, 331216, 331222, 331326, 331331, 331419, 331505, 331544, 332133, 332385, 332905, 332976, 333207, 333225, 333383, 333498, 333748, 333842, 333922, 334139, 334529, 334714, 334742, 334775, 335066, 335076, 335107, 335304, 335362, 335376, 335524, 335525, 335697, 335752, 335758, 335865, 336242, 336267, 336350, 336406, 336503, 336683, 337147, 337156, 337164, 337255, 337445, 337509, 337628, 337689, 337691, 337704, 337808, 337976, 338025, 338214, 338218, 338385, 338819, 338872, 338978, 339051, 339283, 339453, 339579, 339597, 339816, 340129, 340139, 340160, 340535, 340598, 340971, 341039, 341457, 341636, 341737, 342011, 342353, 342374, 342683, 342807, 342963, 342996, 343009, 343158, 343201, 343291, 343598, 343655, 343847, 343968, 343969, 344073, 344196, 344259, 344338, 344399, 345019, 345040, 345062, 345114, 345390, 345781, 345835, 345897, 346026, 346161, 346178, 346250, 346562, 346678, 346712, 346950, 347167, 347407, 347511, 347655, 347908, 347972, 348203, 348277, 348382, 348580, 348639, 348794, 349007, 349038, 349144, 349170, 349212, 349386, 349408, 349663, 350280, 350302, 350500, 350765, 350819, 351134, 351328, 351397, 351566, 351686, 351719, 351759, 351807, 352312, 352357, 352389, 352651, 352814, 352821, 353146, 353200, 353284, 353607, 353893, 353999, 354391, 354445, 354525, 354631, 354690, 354716, 354738, 354791, 355119, 355159, 355223, 355440, 355571, 355593, 355621, 355697, 355717, 355779, 355863, 355922, 356374, 356535, 356569, 356665, 356702, 356916, 356922, 357010, 357272, 357289, 357340, 357508, 357790, 357877, 358029, 358033, 358134, 358223, 358239, 358253, 358289, 358405, 358543, 358706, 358744, 358770, 358788, 358789, 359308, 359323, 359357, 359865, 359868, 360017, 360555, 360570, 360585, 360719, 360759, 360811, 361197, 361685, 361939, 362157, 362247, 362657, 362699, 363190, 363252, 363331, 363363, 363593, 363602, 363671, 363719, 364455, 364467, 364468, 364719, 364913, 365015, 365138, 365314, 365427, 365464, 365659, 365729, 365739, 366009, 366071, 366148, 366313, 366430, 366480, 366795, 366956, 367164, 367357, 367549, 367630, 367716, 367792, 367934, 368363, 368589, 368637, 368833, 369016, 369509, 369735, 369801, 370124, 370152, 370400, 370505, 370524, 370537, 370728, 370790, 370831, 370986, 371029, 371361, 371392, 371486, 371786, 371824, 371871, 371923, 371955, 371960, 372003, 372112, 372156, 372247, 372292, 372309, 372319, 372352, 372558, 372669, 372748, 372871, 373393, 373444, 373645, 373653, 373727, 373730, 374340, 374391, 374818, 375245, 375294, 375331, 375380, 375820, 375996, 376090, 376241, 376258, 376454, 376573, 376750, 376802, 376819, 376838, 376848, 376941, 377007, 377513, 377518, 377570, 377609, 377926, 378586, 378775, 378791, 378916, 379034, 379093, 379136, 379315, 379349, 379434, 379820, 379853, 380122, 380395, 380429, 380440, 380885, 380889, 380949, 381128, 381961, 382005, 382069, 382341, 382469, 382472, 382514, 382620, 382784, 383576, 383605, 383660, 383807, 383917, 383929, 384691, 384745, 384836, 384910, 385337, 385401, 385704, 385882, 386154, 386211, 386401, 386784, 386934, 387105, 387124, 387202, 387256, 387293, 387338, 387365, 387717, 387849, 388403, 388421, 388469, 388894, 388961, 389145, 389154, 389157, 389292, 389498, 389705, 389743, 389772, 390310, 390365, 390474, 390565, 390567, 390663, 390969, 391063, 391175, 391229, 391332, 391439, 391488, 391733, 392167, 392180, 392362, 392657, 392684, 392869, 393095, 393325, 393608, 393629, 394151, 394185, 394447, 395013, 395211, 395221, 395259, 395271, 395425, 395432, 395791, 396014, 396193, 396380, 396536, 396784, 396825, 396933, 397212, 397217, 397390, 397423, 397569, 397760, 398036, 398172, 398305, 398712, 398729, 398872, 398901, 399208, 399276, 399354, 399408, 399432, 399442, 399835, 399922, 400124, 400534, 400740, 401001, 401269, 401455, 401962, 402020, 402041, 402042, 402264, 402298, 402575, 402632, 402806, 402960, 403133, 403197, 403535, 403705, 403841, 403888, 404183, 404205, 404270, 404473, 404475, 404852, 404899, 405013, 405136, 405520, 405582, 405604, 405663, 405709, 406121, 406187, 406230, 406295, 406328, 406988, 407038, 407173, 407246, 407460, 407688, 408163, 408664, 409166, 409454, 409488, 409678, 409754, 409824, 409825, 409918, 410024, 410107, 410165, 410707, 410708, 410916, 410963, 410969, 410992, 411104, 411191, 411238, 411289, 411446, 411778, 411803, 411862, 411877, 412002, 412194, 412691, 412756, 412910, 413088, 413615, 414002, 414850, 415235, 415529, 416076, 416117, 416286, 416355, 416651, 416907, 416948, 417070, 417141, 417220, 417365, 417832, 417844, 418056, 418065, 418500, 418717, 419001, 419019, 419026, 419028, 419110, 419324, 419396, 419599, 419664, 420363, 420366, 420823, 420864, 420892, 421059, 421298, 421596, 422029, 422064, 422255, 422367, 422583, 422782, 422969, 423250, 423341, 423711, 423806, 424068, 424152, 424161, 424193, 424278, 424376, 424408, 424485, 424694, 424844, 425052, 425325, 425628, 425721, 425825, 425945, 426383, 426510, 426551, 426705, 426728, 426829, 426838, 426849, 426877, 426979, 426988, 427169, 427238, 427301, 427362, 427435, 427555, 427628, 427654, 427756, 427779, 427805, 427852, 427853, 427920, 428093, 428576, 428787, 429059, 429437, 429536, 429594, 429959, 430563, 430731, 430889, 430925, 431112, 431178, 431211, 431376, 431704, 432138, 432598, 432615, 432683, 432754, 432897, 433240, 433296, 433398, 433662, 433921, 434201, 434951, 435029, 435272, 435453, 435471, 435869, 436025, 436168, 436620, 436797, 436941, 437080, 437224, 437547, 437632, 438045, 438071, 438099, 438292, 438331, 438429, 438462, 438478, 438663, 438795, 439060, 439273, 439303, 439374, 439509, 439692, 439765, 439889, 439906, 439991, 440002, 440313, 440389, 440511, 440614, 440820, 441205, 441599, 441640, 442062, 442298, 442461, 442680, 443136, 443410, 443455, 443505, 443527, 443562, 443725, 443944, 444033, 444036, 444285, 444344, 444346, 445127, 445276, 445323, 445392, 445405, 445462, 445540, 445689, 446303, 446383, 446539, 446670, 446677, 446726, 446864, 447179, 447424, 447457, 447574, 447681, 447934, 448115, 449158, 449414, 449469, 449780, 450162, 450551, 450707, 450878, 450914, 451119, 451283, 451336, 451337, 451482, 451800, 451818, 451842, 452014, 452229, 452524, 452565, 452619, 452837, 452873, 453002, 453137, 453311, 453553, 453620, 453704, 453906, 453930, 454144, 454174, 454246, 454258, 454406, 454570, 455313, 455406, 455424, 455543, 455649, 455667, 455677, 456176, 456554, 456658, 457085, 457190, 457225, 457286, 457555, 457660, 457976, 458057, 458124, 458172, 458633, 458751, 458762, 458827, 459346, 459465, 459747, 459951, 460139, 460228, 460370, 460442, 461099, 461908, 461996, 462067, 462383, 462445, 462589, 462957, 463224, 463338, 463417, 463474, 463505, 463953, 464166, 464174, 465101, 465200, 465457, 465829, 466024, 466223, 466242, 466523, 466885, 467774, 467905, 468117, 468219, 468401, 468465, 468518, 468760, 469293, 469427, 469545, 469559, 469567, 469658, 469825, 469832, 470004, 470072, 470085, 470174, 470393, 470501, 470893, 470976, 470977, 471096, 471136, 471315, 471332, 471665, 471698, 471962, 471966, 472506, 472654, 472749, 472954, 473003, 473072, 473348, 473352, 473373, 473500, 473879, 474123, 474342, 474424, 474461, 474699, 474725, 475007, 475037, 475129, 475236, 475533, 475651, 475754, 475988, 476060, 476347, 476934, 477005, 477040, 477266, 477392, 477580, 477590, 477797, 478105, 478148, 478164, 478712, 478833, 478892, 478899, 479168, 479172, 479396, 479707, 479886, 480014, 480196, 480240, 480576, 480741, 480779, 480843, 480908, 481165, 481218, 481292, 481355, 481428, 481530, 481609, 481736, 481804, 482093, 482195, 482251, 482326, 482330, 482454, 482472, 482706, 482731, 482775, 483015, 483078, 483261, 483363, 483611, 483766, 484108, 484206, 484208, 484307, 484369, 484385, 484620, 485016, 485306, 485364, 485367, 485602, 485632, 485705, 485757, 485800, 485954, 485984, 486300, 486606, 486713, 486936, 487009, 487264, 487284, 487464, 487502, 487510, 487602, 487806, 487992, 488073, 488139, 488404, 488641, 489107, 489145, 489695, 489971, 490016, 490182, 490356, 490490, 490507, 490887, 491204, 491249, 491273, 491477, 491666, 491707, 491739, 492040, 492138, 492155, 492219, 492268, 492293, 492302, 492408, 492638, 492894, 493504, 493626, 493936, 494032, 494128, 494174, 494257, 494534, 494706, 495233, 495528, 495776, 496053, 496261, 496374, 496457, 496732, 496752, 496839, 497296, 497311, 498297, 498508, 498639, 498669, 498679, 498706, 498730, 498854, 499122, 499141, 499155, 499538, 499682, 499738, 499966, 500057, 500214, 500440, 500561, 500594, 500603, 500686, 501269, 501710, 501842, 502015, 502134, 502148, 502300, 502407, 502470, 502553, 502679, 502726, 503022, 503478, 503497, 503500, 503541, 503777, 504211, 504259, 504554, 504616, 504744, 504748, 504769, 505288, 505884, 505885, 505895, 505898, 505924, 506030, 506056, 506162, 506226, 506231, 506592, 506740, 506837, 507073, 507215, 507266, 507342, 507642, 507761, 507765, 507776, 507815, 507952, 508140, 508200, 508311, 508429, 508456, 508467, 508504, 509039, 509269, 509555, 509652, 509746, 510342, 510493, 510572, 510617, 510860, 510976, 510977, 511036, 511146, 511580, 511642, 511930, 511967, 512282, 512400, 512458, 512644, 512658, 512951, 513221, 513683, 513811, 514064, 514213, 514230, 514243, 514295, 514391, 514435, 514559, 514622, 515229, 515401, 515470, 515512, 515590, 515623, 515702, 515815, 516106, 516263, 516481, 516791, 516906, 516990, 517403, 517451, 517492, 517685, 517805, 517869, 517920, 517985, 518215, 518552, 518785, 518918, 518966, 519205, 519477, 519616, 519626, 520100, 520112, 520199, 520272, 520445, 520456, 520479, 520767, 520883, 521064, 521184, 521338, 521366, 521437, 521514, 521618, 521709, 522062, 522074, 522191, 522240, 522288, 522342, 522365, 522416, 522423, 522462, 522465, 522704, 522771, 522947, 523484, 523487, 523561, 523577, 523795, 523995, 524155, 524227, 524340, 524369, 524476, 524520, 524662, 524866, 524966, 524991, 525342, 525555, 526029, 526070, 526521, 526523, 526552, 526597, 526695, 526713, 526769, 526912, 527073, 527139, 527267, 527345, 527597, 527796, 527822, 527925, 528020, 528071, 528198, 528493, 528851, 528941, 528970, 528992, 529016, 529345, 529376, 529624, 530097, 530132, 530406, 530629, 530903, 531201, 531277, 531388, 531444, 531550, 531752, 531834, 532335, 532376, 532595, 532622, 532711, 533050, 533218, 533220, 533827, 533897, 534037, 534155, 534166, 534224, 534311, 534440, 534543, 534711, 535049, 535101, 535218, 535229, 535234, 535289, 535358, 535418, 535561, 535666, 535874, 536039, 536127, 536146, 536244, 536278, 536555, 536576, 536730, 536820, 536823, 536902, 536960, 537371, 537461, 537553, 537720, 537770, 537807, 537960, 538196, 538263, 538398, 538537, 538544, 538574, 538633, 538737, 538805, 539158, 539475, 539632, 539851, 539941, 540370, 540436, 541255, 541338, 541472, 541938, 541949, 542027, 542160, 542173, 542442, 542718, 542799, 542936, 542988, 543233, 543617, 543642, 543790, 543833, 543838, 543882, 543947, 544109, 544169, 544294, 544831, 544875, 545022, 545145, 545213, 545214, 545260, 545325, 545351, 545411, 545721, 545793, 545850, 546046, 546093, 546218, 546242, 546408, 547055, 547165, 547315, 547348, 547411, 547974, 548136, 548416, 548575, 548772, 549127, 549366, 549599, 549605, 550129, 550134, 550140, 550308, 550311, 550354, 550532, 550726, 550844, 550972, 551172, 551197, 551244, 551316, 551472, 551524, 551607, 551793, 551814, 551869, 551873, 552184, 552199, 552272, 552291, 552549, 553126, 553176, 553308, 553498, 553586, 554031, 554168, 554598, 554699, 554703, 554950, 555022, 555120, 555654, 555771, 555794, 556162, 556176, 556399, 556424, 556544, 556698, 556830, 556888, 557602, 557628, 557678, 557694, 557746, 558276, 558372, 558804, 558824, 558890, 559132, 559267, 559271, 559497, 559618, 559700, 559760, 559830, 560152, 560155, 560180, 560372, 560517, 560532, 560576, 560809, 560909, 561028, 561339, 561384, 561454, 561479, 561582, 561593, 561818, 562063, 562092, 562100, 562162, 562826, 563110, 563364, 563525, 563545, 563658, 564063, 564228, 564271, 564349, 564449, 564508, 564823, 565220, 565243, 565476, 565608, 565664, 565769, 565884, 566245, 566301, 566319, 566592, 566612, 566968, 567189, 567396, 567566, 567937, 567964, 568272, 568654, 568725, 568788, 568840, 568851, 569214, 569234, 569255, 569261, 569286, 569769, 569795, 569851, 570178, 570211, 570285, 570581, 570656, 570878, 571563, 571654, 571658, 571661, 571671, 571694, 571702, 571719, 572179, 572307, 572353, 572529, 572602, 572689, 572732, 572786, 572801, 572949, 572998, 573476, 573632, 573704, 573825, 573875, 573961, 574251, 574299, 574368, 574420, 574443, 574563, 574760, 574870, 574957, 574961, 574983, 575049, 575417, 575461, 575519, 575980, 576153, 576157, 576286, 576543, 576581, 576829, 577126, 577140, 577197, 577399, 577405, 577416, 577558, 577583, 577725, 577850, 578002, 578294, 578369, 578519, 578523, 578567, 578702, 578805, 578808, 579057, 579255, 579299, 579440, 579667, 580008, 580238, 580374, 580668, 580695, 580785, 580905, 580957, 581282, 581518, 581563, 581766.


==> tbls/holistic_abl.tex <==
\begin{table}[!t]
\centering
\resizebox{0.6\textwidth}{!}{
    \begin{tabular}{lcccc}
        \hline
        \textbf{MODEL} & CLS(\%) & CAP (CIDEr) & VQA(\%) & GQA(\%) \\
        \hline
        Con          & 91.3          & 104.4          & 68.5          & 55.3 \\
        Cap          & 90.4          & 107.1          & 70.9          & 58.5  \\
        CapPa        & \textbf{90.9} & 107.6          & 70.9          & 58.3 \\
        \modelname{} & 90.1          & \textbf{107.8} & \textbf{72.0} & \textbf{61.7} \\
        \hline
    \end{tabular}}
\caption{Ablation study on holistic tasks.}
\label{tbl:hol_resuls_abl}
\end{table}


==> tbls/pali_eval_G.tex <==
\begin{table}[h]
\centering
\caption{\modelname{}$_G$ outperforms SigLIP$_G$ significantly on the same PaLI-3~\cite{chen2023pali3} transfer tasks.}
 \scriptsize
\begin{tabularx}{\linewidth}{>{\hsize=1.0\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X}
\toprule
\textbf{MODEL} & COCO & VQAv2 & OKVQA & TextVQA & ST-VQA & TallyQA \\
\hline
\modelname{}$_L$ & 138.9 & 77.6 & 58.4 & 49.2 & 50.9 & 79.3/64.1 \\
SigLIP$_G$ & 140.3 & 77.5 & 58.6 & 50.6 & 50.5 & 76.3/61.8 \\
\modelname$_G$ & \textbf{140.9} & \textbf{78.1} & \textbf{59.8} & \textbf{52.1} & \textbf{52.3} & \textbf{79.0/64.2} \\
\bottomrule
\end{tabularx}
\label{tbl:pali_eval_G}
\end{table}

==> tbls/refcoco_abl.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{0pt}
\setlength{\extrarowheight}{5pt}
\renewcommand{\arraystretch}{0.75}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\centering \scriptsize
\caption{Comparison with baselines on RefCOCOs. A randomly initialized decoder is trained for REC, keeping the image representation is frozen. Here CLIP uses model checkpoints released by~\cite{clip}; all other baselines are trained on the same data as \modelname{}.}
\label{tbl:refcoco_abl}
% \vspace{-2mm}
\begin{tabularx}{\linewidth}{>{\hsize=1.0\hsize}X>{\hsize=.6\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X}
 \toprule[1pt]
\multirow{2}{*}{\textbf{MODEL}} & \multicolumn{3}{c}{RefCOCO} \hspace{15pt} & \multicolumn{3}{c}{RefCOCO+} \hspace{5pt} & \multicolumn{2}{c}{RefCOCOg} \hspace{15pt} \\
\cmidrule(r{15pt}){2-4} \cmidrule(l{0pt}r{16pt}){5-7} \cmidrule(l{0pt}r{11pt}){8-9}
& val & testA & testB & val & testA & testB & val-u & test-u \\
    \midrule
\textcolor{gray}{CLIP}~\cite{clip}  &                \textcolor{gray}{\underline{65.21}} &              \textcolor{gray}{\underline{71.28}} &              \textcolor{gray}{58.17} &                 \textcolor{gray}{\underline{57.53}} &               \textcolor{gray}{\underline{66.44}} &               \textcolor{gray}{47.77} &                 \textcolor{gray}{\underline{59.32}} &              \textcolor{gray}{\underline{60.24}} \\
CLIP* &                58.28 &              63.59 &              53.73 &                 49.01 &               55.94 &               41.96 &                 55.70 &              55.88 \\
Cap~\cite{cappa}  &                60.64 &              65.47 &              56.17 &                 52.56 &               58.32 &               45.99 &                 56.75 &              57.99 \\
CapPa~\cite{cappa} &                64.17 &              69.90 &              \underline{58.25} &                 56.14 &               63.68 &               \underline{48.18} &                 58.90 &              59.91 \\
\arrayrulecolor{lightgray}
\midrule[0.25pt]\arrayrulecolor{black}
LocCa &                \textbf{88.34} &              \textbf{91.20} &              \textbf{85.10} &                 \textbf{79.39} &               \textbf{85.13} &               \textbf{72.61} &                 \textbf{81.69} &             \textbf{82.64}\\
\bottomrule
\end{tabularx}
% \vspace{-2mm}
\end{table*}


==> tbls/refcoco_tok_res_abl.tex <==
\begin{table*}[!t]
  \centering
  \caption{Ablation studies on string (Str.) vs special (Spec.) tokenization for box coordinates and impact on image resolution.}
  \label{tbl:refcoco_tok_res_abl}
\begin{tabularx}{\linewidth}{>{\hsize=0.7\hsize}X>{\hsize=1.4\hsize}X>{\hsize=.7\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X}
    \toprule
    \multirow{2}{*}{Tok.} & \multirow{2}{*}{Res.} & \multicolumn{3}{c}{RefCOCO} & \multicolumn{3}{c}{RefCOCO+} & \multicolumn{2}{c}{RefCOCOg} \\
    \cmidrule(r){3-5} \cmidrule(lr){6-8} \cmidrule(l){9-10}
     & & val & testA & testB & val & testA & testB & val-u & test-u \\
    \midrule
Str. & 224 -> 224                     & 90.3   & 93.3   & 87.7  & 84.1   & 89.5   & 78.9   & 84.5 & 86.0  \\
Str. & 224 -> 384                     & 91.1   & \underline{94.0}   & 88.7  & 85.6   & 90.9   & 79.8  & 86.7 & 87.4  \\
Str. & 224 -> 640                     & \textbf{91.9}   & \textbf{94.6}   & \textbf{89.1}  & \textbf{86.5}   & \textbf{91.7}   & \underline{80.4}  & \underline{87.5} & \underline{88.0}  \\
Spec. & 224 -> 224                     & 90.6   & 92.9   & 87.3  & 83.9   & 88.0   & 78.4 &  84.9 & 86.0  \\
Spec. & 224 -> 384                     & 90.9   & 93.5   & 87.9  & 86.0   & 90.5   & 79.5   & 86.4 & 87.8 \\
Spec. & 224 -> 640                     & \underline{91.4}   & 93.8   & \underline{88.9}  & \underline{86.1}   & 90.6   & \textbf{80.8}   & \textbf{87.8} & \textbf{88.2} \\
\bottomrule
\end{tabularx}
\end{table*}


==> tbls/refcocoseg_abl.tex <==

\begin{table*}[ht]
\setlength{\tabcolsep}{0pt}
\setlength{\extrarowheight}{5pt}
\renewcommand{\arraystretch}{0.75}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\centering \scriptsize
\caption{mIoU on RefCOCO \textbf{segmentation} for different pretrained, frozen vision encoders (ViT-L/14). The decoders are trained from scratch for all models to ensure a fair comparison. The LocCa vision encoder outperforms other encoders substantially.}
\label{tbl:refcocoseg_abl}
% \vspace{-2mm}
\begin{tabularx}{\linewidth}{>{\hsize=1.0\hsize}X>{\hsize=.6\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X}
 \toprule[1pt]
\multirow{2}{*}{\textbf{MODEL}} & \multicolumn{3}{c}{\hspace{15pt} RefCOCO}  & \multicolumn{3}{c}{RefCOCO+ \hspace{15pt}}  & \multicolumn{2}{c}{RefCOCOg \hspace{15pt}} \\
\cmidrule(r{15pt}){2-4} \cmidrule(l{0pt}r{16pt}){5-7} \cmidrule(l{0pt}r{11pt}){8-9}
& val & testA & testB & val & testA & testB & val-u & test-u \\
    \midrule

\textcolor{gray}{CLIP~\cite{clip}} &
\textcolor{gray}{36.15} & \textcolor{gray}{38.25} & \textcolor{gray}{35.82} & \textcolor{gray}{31.40} & \textcolor{gray}{36.00} & \textcolor{gray}{28.69} & \textcolor{gray}{29.21} & \textcolor{gray}{29.44} \\

CLIP* &
32.78 & 34.89 & 33.03 & 27.49 & 30.14 & 25.07 & 26.99 & 26.83 \\

Cap~\cite{cappa} &
34.84 & 37.68 & 35.39 & 31.93 & 35.24 & 28.79 & 28.84 & 29.11 \\

CapPa~\cite{cappa} &
36.62 & 39.23 & 36.67 & 32.54 & 37.49 & 29.59 & 30.40 & 30.43 \\

\arrayrulecolor{lightgray}\midrule[0.25pt]\arrayrulecolor{black}

LocCa &
64.98 & 65.39 & 64.09 & 57.85 & 60.92 & 52.72 & 55.84 & 56.95 \\

\bottomrule
\end{tabularx}
% \vspace{-2mm}
\end{table*}

